Probabilistic Implicit Scene Completion

We propose a probabilistic shape completion method extended to the continuous geometry of large-scale 3D scenes. Real-world scans of 3D scenes suffer from a considerable amount of missing data cluttered with unsegmented objects. The problem of shape completion is inherently ill-posed, and high-quality result requires scalable solutions that consider multiple possible outcomes. We employ the Generative Cellular Automata that learns the multi-modal distribution and transform the formulation to process large-scale continuous geometry. The local continuous shape is incrementally generated as a sparse voxel embedding, which contains the latent code for each occupied cell. We formally derive that our training objective for the sparse voxel embedding maximizes the variational lower bound of the complete shape distribution and therefore our progressive generation constitutes a valid generative model. Experiments show that our model successfully generates diverse plausible scenes faithful to the input, especially when the input suffers from a significant amount of missing data. We also demonstrate that our approach outperforms deterministic models even in less ambiguous cases with a small amount of missing data, which infers that probabilistic formulation is crucial for high-quality geometry completion on input scans exhibiting any levels of completeness.

==> 03_cgca_neurips.tex <==
\section {Continuous Generative Cellular Automata}
\begin{figure}[t]
	\includegraphics[width=0.95\textwidth]{./figures/method_overview.pdf}
	\centering

	\caption[] {
	    Overview of our method.
	    Our method is composed of two stages: stochastic voxel generation (left) and implicit function reconstruction (right).
	    The first stage follows the Markov chain of the transition kernel $p_\theta$ to progressively generate a sparse set of occupied voxels. The second stage observes the voxels $s^T$ and associated features $e^T$, and produces an implicit function value $\hat{d}_q=f_\omega(\Psi (g_{\phi}(s^T, e^T), q))$ at the query point location $q$ by aggregating hierarchical features $g_\phi(s^T, e^T)=F_1, \ldots, F_n$.
	    }
	\label{fig:method_overview}
\end{figure}

In this section, we introduce how continuous implicit surface can be produced in conjunction with the sparse occupied voxels from GCA.
Then, we explain the training algorithm and prove that the training of stochastic generation maximizes the lower bound of the data distribution, which justifies the theoretical aspect as a valid generative model.


\subsection{Reconstructing Implicit Surfaces from Sparse Voxels}

We formulate the reconstruction problem as a two-step procedure: (i) stochastic voxel generation and (ii) implicit function reconstruction.
The overall procedure is depicted in Figure~\ref{fig:method_overview}.
The stochastic generation of the sparse voxels directly follows the formulation of GCA~\cite{zhang2021gca}.
Basically, we repeat the $T$ steps of sampling from the aggregated transition kernel in Equation~(\ref{eq:cell_sampling}) to progressively grow the shape.
Then the state $s^T$ is transformed into an implicit surface by evaluating the distance value for each query point $q \in \mathbb{R}^3$.
Note that an efficient sampling of query points near the surface is possible by sampling near the sparse voxel, which is already an approximation of the surface.
The final reconstruction is the implicit representation created from $s^T$.

The implicit function reconstruction is composed of the encoder $g_\phi$ and the decoder $f_\omega$.
The encoder receives $s^T$ sampled from the voxel generation step using the formulation of GCA.
In addition, the transition kernel $p_\theta$ outputs the $K$ dimensional feature $l_c \in \mathbb{R}^K$ for each occupied cell $c \in s^T$, which is consumed as the auxiliary feature $e^T=\{l_c\in \mathbb{R}^K\mid c \in s^{T}\}$ for the encoder.
The encoder $g_\phi$ transforms the sparse set of the coordinate-feature pairs $(s^T, e^T)$ into the hierarchical feature representation that summarizes the local context of each grid cell.
Then the decoder $f_\omega$ regresses the distance values~\cite{chibane20ifnet,peng2020conv_onet} using the information from the encoded feature $g_\phi(s^T, e^T)$.
Note that we intentionally re-use the deep sparse CNN for the transition kernel $p_\theta$ to train the entire network in an end-to-end fashion.

The right side of Figure~\ref{fig:method_overview} illustrates the implicit surface reconstruction module.
The encoder $g_\phi$ aggregates the information into multi-level grids in $n$ different resolutions
\begin{equation}
	g_\phi(s^{T}, e^{T}) = F_1, F_2, ..., F_{n},
\end{equation}
similar to IF-Net~\cite{chibane20ifnet}.
Starting from the original resolution $F_1$, $F_k$ contains a grid that is downsampled $k$ times.
However, in contrast to the original IF-Net, our grid features are sparse, since they only store the downsampled occupied cells of state $s^T$.
The sparse representation $F_k = (s_k, e_k)$ is composed of coordinates $s_k \subset \mathbb{Z}^3$ and  $L$-dimensional features $e_k = \{l_{c} \in \mathbb{R}^L \mid c \in s_k \}$.
The grid points that are not in $s_k$ are considered as having zero features.
Throughout the paper, we use $n=3$ levels.

The feature for a query point $q$ is obtained via adding all the multi-scale features: $\Psi (g_{\phi}(s^T, e^T), q) = \sum_k \psi_k(F_k, q)$. %
At the $k$-th scale, the feature at a particular position $q$ is evaluated by trilinear interpolation  $\psi_k(F_k, q) \in \mathbb{R}^L$ of the feature $F_k$ at $k$-th level grid as in IF-Net~\cite{chibane20ifnet}.
The decoder $f_\omega: \mathbb{R}^L \rightarrow \mathbb{R}$ is an MLP that maps the feature at the query point 
$\Psi (g_{\phi}(s^T, e^T), q)$
to the implicit function value $\hat{d}_q$.
We use truncated signed distance within the range of $[-1,1]$.
Note that we can also use unsigned distance function as in NDF~\cite{chibane2020ndf} by changing the codomain of the decoder to $[0, 1]$.

While the sampling procedure in Equation~(\ref{eq:transition_kernel}) enables efficient multi-modal shape generation, the output needs to converge to the single coherent shape at the final step.
However, na\"i\ve sampling can produce blurry shapes when few voxels with low-occupancy probability are included.
As a simple trick, we augment \textit{mode seeking steps}. 
During the mode seeking steps, we run a few additional $T'$ steps of the transition kernel but we select the cells with probability higher than 0.5 instead of implementing stochastic sampling.
The mode seeking steps prevent the cells with low probability from being sampled and the final continuous surface of the shape converges to a single mode that is closest to $s^T$.
The effects of mode seeking steps are visualized in Appendix~\ref{appendix:mode_seeking_steps}.



\subsection{Training Continuous Generative Cellular Automata}
\label{sec:training_cgca}

Since cGCA is composed of two modules, stochastic voxel generation and implicit function reconstruction, we introduce the training procedure of each module separately.

\paragraph{Stochastic Voxel Generation.}
At training time, we aim to learn the parameters $\theta$ of the transition kernel $p_\theta(s^{t + 1} \mid s^t)$, whose finite number of applications yields the samples from the learned distribution.
The training data contains an initial incomplete state $s^0$ and complete state $x$, which represents the surface as sparse voxels for each data.
Since we are given only the initial and final state, we need to emulate the sequence by using infusion training~\cite{bordes2017infusion}, which induces the chain to converge to the complete state.
To do so, we define a function $G_x(s)$ that finds the state that is closest to the complete state $x$ from the current state $s$ within the neighborhood $\mathcal{N}(s)$:
\begin{equation}
		G_x(s) = \{\mathrm{argmin}_{c \in \mathcal{N}(s)}  d(c, c') \mid c' \in x\}.
\end{equation}
Then, we define the infusion kernel $q^t$:
\begin{equation}
    \quad q^t_\theta(s^{t+1} \mid s^t, x) = \prod_{c \in \mathcal{N}(s^t)} (1 - \alpha^t) p_\theta(c \mid s^t) + \alpha^t \delta_{G_x(s^t)}(c),
\end{equation}
where $\delta_{G_x(s^t)}(c)$ is formulated as Bernoulli distribution with probability 1, if $c \in G_x(s^t)$, else 0.
$\alpha^t$ is the infusion rate set to increase linearly with respect to time step, i.e., $\alpha^t = \max(wt + \alpha_0, 1)$, with $w > 0$.
Thus the infusion kernel for each cell is defined to be a mixture of $p_\theta$ and $\delta_{G_x(s^t)}$, where $\delta_{G_x(s^t)}$ is crucial to guarantee that the sequence ultimately reaches the ground truth shape.
The following proposition proves that the infusion chain converges to the complete data in a finite number of steps.

\begin{restatable}{prop}{infusionconvergence} \label{prop:infusion_convergence}
		If the infusion rate $\alpha^t$ increases until it reaches a maximum value of 1 and every state $s^t$ is non-empty, then there exists $T$ such that $s^T = x$.
	\label{prop1}
\end{restatable}
\begin{proof}
	\vspace{-0.7em}
	The proof is found in Appendix~\ref{appendix:prop1}.
	\vspace{-0.7em}
\end{proof}

Thus, the training procedure for each step $s^t$ is to sample $s^{t + 1} \sim q_\theta(\cdot \mid s^t)$ and minimize the negative log-likelihood of its next state $s^{t + 1}$ 
\begin{equation}
    \mathcal{L_{\textit{voxel}}} = - \log p_\theta(s^{t + 1} \mid s^t).
    \label{eq:loss_voxel}
\end{equation}

While the training procedure of the voxel generation is similar to that of GCA, our voxel generation module is more flexible in the aspect that we do not assume any connectivity of the shape for convergence.
Instead, the infusion using the auxiliary function $G_x(s)$ ensures the convergence which is further verified in Appendix~\ref{appendix:gca_comparison}.
Also, while the likelihood objective of GCA is based on heuristics, our objective can be shown to maximize the lower bound of the log-likelihood of the complete state shown in Section~\ref{sec:lower_bound_derivation}.

\paragraph{Implicit Function Reconstruction.}
To train the network that regresses continuous surface, we train the neural network with a set $Q = \{(q, d_q)| q\in\mathbb{R}^3\}$, where $q$ is the points near the surface and $d_q$ is the signed distance from the surface to query point.
Since the voxel generation progressively completes the sparse voxels as if it were expanding the surface, we train the network to reconstruct the voxels for every state $s^t$ during the training step.
The loss function is defined as 
\begin{equation}
	\mathcal{L_{\textit{implicit}}} = \sum_{q \in Q} |f_w(\Psi (g_{\phi}(s^T, e^T), q)) - \max(\min(\frac{d_q}{\epsilon}, 1), -1)|,
	\label{eq:loss_implicit} 
\end{equation}
where $s^{t + 1}$ and $e^{t + 1}$ are sampled from the transition kernel $p_\theta$ and $\epsilon$ is the size of a single voxel.
Clamping the maximum distance lets the network focus on  accurately predicting in the vicinity of the surface~\cite{park2019deepsdf, chibane2020ndf}.
 
To summarize, the total loss $\mathcal{L_{\textit{total}}}$ at state $s^t$ is the weighted sum of $\mathcal{L_{\textit{voxel}}}$ and $\mathcal{L_{\textit{implicit}}}$:
\begin{equation}
	\mathcal{L_{\textit{total}}} = \mathcal{L_{\textit{voxel}}} + \beta \mathcal{L_{\textit{implicit}}},
	\label{eq:loss_total}
\end{equation}
where $\beta$ is a  hyperparameter.
To stabilize the training regardless of the varying level of incompleteness, the full training algorithm normalizes the loss function with the number of occupied voxels and utilizes a data buffer to control the length of the transition steps~\cite{zhang2021gca}.
The details of the end-to-end training can be found in Appendix~\ref{appendix:implementation_details}.



\subsection {Derivation of Maximizing Lower Bound of Log-likelihood}
\label{sec:lower_bound_derivation}


In this section, we verify that the training objective leads to a valid generative model.
The derivation focuses only on the final generated shape instead of the intermediate steps in the Markov chain.
We show that the process indeed maximizes the lower bound for the marginal log-likelihood of the complete state that we want to achieve at the last step.


We first use Proposition~\ref{prop:infusion_convergence} to find $T$ such that $x = s^T$, inducing $\log p_\theta(x) = \log p_\theta(s^T)$.
However, since the direct optimization of the exact log-likelihood is intractable, we show that our training objective in Equation~(\ref{eq:loss_voxel}) maximizes its variational lower bound, using the derivation from Luo \& Hu~\cite{luo2021diffusion}:

\begin{align}
	\log p_\theta(s^T) 
	&\ge \sum_{s^{0: T-1}} q_\eta(s^{0:T-1}|s^T) \log \frac{p_\theta(s^{0:T})}{q_\eta(s^{0:T-1}|s^T)} \\
	&= \log \frac{p(s^0)}{q(s^0)} + \E_{q_\eta}[\log p_\theta(s^T | s^{T - 1})] - \sum_{0 \le t < T - 1} D_{KL}(q_\eta(s^{t + 1} | s^t, s^T) \| p_\theta(s^{t + 1} | s^t))) 
	\label{eq:elbo}
\end{align}
where the full derivation is in Appendix~\ref{section:detailed_derivation} for the reader's convenience.
The parameter $\eta$ of $q$ is substituted with $\theta$ every time $\theta$ is updated. 
Note that the first term of Equation~(\ref{eq:elbo}) has no trainable parameters and the second term is maximized directly from the training objective.
The following proposition shows that the training objective minimizes the third KL divergence term, therefore maximizing the log-likelihood of data distribution.

\begin{restatable}{prop}{maximizinglowerbound} \label{prop:maximizing_lower_bound}
	If the likelihood for every cell $c \in s^{t + 1}$ increases when updating parameters $\theta$ with $\theta'$ by minimizing Equation~\text{(\ref{eq:loss_voxel})}, where $s^{t + 1} \sim q_\theta(\cdot | s^t)$, i.e., $ p_{\theta'}(c | s^t) \ge p_{\theta}(c | s^t), \; \forall c \in s^{t+1}$, then the KL-divergence term in Equation~\text{(\ref{eq:elbo})} decreases, i.e., $D_{KL}(q_{\theta'}(s^{t + 1} | s^t, s^T) \| p_{\theta'}(s^{t + 1} | s^t)) \le D_{KL}(q_{\theta}(s^{t + 1} | s^t, s^T) \| p_{\theta}(s^{t + 1} | s^t))$.
\end{restatable}
\begin{proof}
	\vspace{-0.7em}
	The proof is found in Appendix~\ref{appendix:prop2}.
	\vspace{-0.7em}
\end{proof}

Thus, the lower bound of the marginal log-likelihood is maximized.


==> 04_exp_neurips.tex <==
\section{Experiments}

We test the probabilistic shape completion for a single object (Section~\ref{sec:single_object_completion}) and scene (Section~\ref{sec:scene_completion}) dataset.
Details regarding the hyperparameters and baselines are in Appendix~\ref{appendix:implementation_details}.


\subsection{Single Object Completion}
\label{sec:single_object_completion}


The single object probabilistic completion with cGCA is compared against cGAN~\cite{wu2020msc} and GCA~\cite{zhang2021gca}.
We use the shapes of chair, sofa, and table category from ShapeNet~\cite{chang2015shapenet} dataset which are normalized to fit within a unit sphere.
For training cGCA, we obtain the query points with corresponding signed distance values from watertight mesh as in DeepSDF~\cite{park2019deepsdf}.
The partial input is generated by first uniformly sampling the mesh and then extracting points within a sphere of radius 0.5, centered at one of the surface points.
Then we sample 1,024 points to create a sparse input.
For GCA and cGCA, we create a quantized version of the sparse voxel grid by placing the point cloud into a grid and marking cells containing points as occupied.

We generate ten completions for each input and compare the performance in terms of three metrics: minimal matching distance (MMD), unidirectional Hausdorff distance (UHD), and total mutual distance (TMD) by following the work of Wu et al.~\cite{wu2020msc}.
The metrics are calculated using point cloud, which is the output of cGAN. 
The output of GCA is a set of occupied voxels which are turned into a mesh with marching cubes~\cite{lorensen1987mcubes} and then sampled.
The points of the implicit representation of cGCA are extracted from positions where the regressed distance value is below half of the grid length.

\input{table/result_shapenet}
\begin{figure}[t]
    \vspace{-0.5em}
	\includegraphics[width=\textwidth]{./figures/single_object_comparison.pdf}
	\centering

	\caption[] {
	    Qualitative comparison on single object completion against cGAN~\cite{wu2020msc} and GCA~\cite{zhang2021gca}
	}
	\label{fig:single_object_comparison}
\end{figure}




The superior performance of cGCA is reported in Table~\ref{table:single_object_completion_comparison}.
Since the number of generated points in cGAN is fixed to 2,048, we first compare by sampling 2,048 points (top of Table~\ref{table:single_object_completion_comparison}) and once again sampling 16,384 points without cGAN to examine the high resolution surface (bottom).
Our method in signed representation outperforms all other methods in MMD (quality) and UHD (fidelity) in average, while having comparable TMD (diversity) against GCA.
This indicates that cGCA generates shapes close to the data distribution (MMD) while being diverse (TMD) and faithful to the input (UHD).
Figure~\ref{fig:single_object_comparison} shows that cGCA is able to generate a smooth surface while other works are either limited to the number of points or the voxel resolution.

To show that cGCA can generate surfaces beyond the voxel resolution, we compare the results of GCA and cGCA in two different voxel resolutions, $32^3$ and $64^3$.
The voxel resolution affects the estimation accuracy of the true surface of the shape, as compared in Figure~\ref{fig:single_object_ablation}.
Table~\ref{table:single_object_completion_comparison} shows that both GCA and cGCA achieve better performance in all three metrics at $64^3$ voxel resolution.
The difference is less prominent for cGCA, and signed cGCA clearly outperforms GCA of the same resolution in terms of MMD and UHD.
Notably, cGCA of voxel resolution $32^3$ shows better results in MMD than GCA in voxel $64^3$ resolution, thereby showing the expressive power of the implicit representation beyond the voxel resolution.


We also show the results using unsigned distance fields as in NDF~\cite{chibane2020ndf} in place of signed distance fields for the implicit representation.
While signed representation can only represent closed surfaces, the unsigned implicit field is applicable to mesh with various topology.
However, the flexibility comes at the cost of expressive power, achieving higher MMD and UHD compared to the signed counterparts.
Without a clear distinction between the interior/exterior, the unsigned representation also makes it difficult to scrutinize the zero-level isosurface and thus results in comparably thick chair legs as shown in Figure~\ref{fig:single_object_ablation}.
Nonetheless, the unsigned cGCA outperforms MMD scores compared to that of GCA, which indicates that it generates surface beyond the voxel resolution.

\subsection{Scene Completion}
\label{sec:scene_completion}


\input{table/result_synthetic}


\begin{figure}[t]
	\includegraphics[width=\textwidth]{./figures/fig3_synthetic}
	\centering
	\caption[] {
	    \TODO{Write caption}
	}
	\label{fig:synthetic_comparison}
\end{figure}



\input{table/result_3dfront}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.97\textwidth]{./figures/scene_completion_comparison.pdf}

	\caption[] {
	    Qualitative comparison on probabilistic scene completion.
	    Best viewed on screen.
	    Since the raw inputs of furniture are highly incomplete, there exists multiple plausible reconstructions.
	    Probabilistic approaches produce diverse yet detailed scene geometry.
	    GCA suffers from artifacts due to the discrete voxel resolution.
	    \TODO{change figure}
	    \vspace{-1.5em}
	}
	\label{fig:scene_comparison}
\end{figure}



Probabilistic scene completion is tested with 3DFront~\cite{fu20203dfront} synthetic scene dataset.
We sample 7891 and 1917 rooms for training and validation set, respectively.
The unsigned distance value is sampled in the vicinity of mesh, whose positions are randomly perturbed from the surface with Gaussian noise.
The partial input is created by first sampling surface points and then iteratively removing points  within a fixed distance from a random position for each object in the scene.
The partial input for multi-modal scene completion is guaranteed to maintain at least 30\% of initial points sampled from the original surface.
Lastly, the input points are voxelized with size 5cm and 20\% of the voxels are removed for a sparse input.
The sparse and incomplete input encourages diverse outputs as shown in Figure~\ref{fig:scene_comparison}.
Further details about the data preparation are articulated in Appendix~\ref{appendix:data_preparation}.



Note that the scenes are composed of multiple pieces of mesh, and cannot be processed with previous works that utilize signed distance field~\cite{peng2020conv_onet, chibane20ifnet, chiyu2020local}.
To employ signed distance field, it is necessary to convert the input to a watertight mesh with pre-processing, which is especially challenging when the 3D model is obtained from a noisy scan.
Being able to handle unsigned distance fields, our approach can be readily applied in scenes, where the inherent scalability of cGCA can be fully exploited.


We compare our method against NDF~\cite{chibane2020ndf} and GCA~\cite{zhang2021gca}.
NDF uses the implicit representation based on unsigned distance field as ours, but produces deterministic completion.
GCA, on the other hand, is capable of generating multi-modal outcomes, but uses discretized representation with voxels.
For probabilistic methods, we generate five completions and sample points proportional to the size of the room.
We introduce min-Chamfer-\textit{L}1, average-Chamfer-\textit{L}1 metrics, which compare the minimum and average of Chamfer distance of outcomes to the ground truth mesh.
We also evaluate TMD and UHD.

The quantitative results are shown in Table~\ref{table:scene_completion_comparison}.
Our method achieves high TMD scores, implying that we can generate diverse high-quality surfaces.
Despite the diversity, the outcome is still similar to the ground truth with a low Chamfer-\textit{L}1 distance.
As demonstrated in single object completion, the network with unsigned distance function thickens some fine details, and our UHD scores are slightly higher than that of GCA.
However, the visual quality shown in Figure~\ref{fig:scene_comparison} clearly indicates that  GCA suffers from discretization artifact of voxels whereas cGCA can generate continuous surfaces.

Our results further verify the discussion by Goodfellow~\cite{goodfellow2017gan_tutorial}: generative models need to capture multi-modal distribution, as deterministic models can merely estimate the mean value of complex multiple possibilities and generate blurry outputs.
As shown in Figure~\ref{fig:scene_comparison} and Table~\ref{table:scene_completion_comparison}, the deterministic method (NDF) fails to generate plausible scenes when the input scene is largely incomplete.
On the other hand, the probabilistic methods (GCA and cGCA) successfully recover a single mode despite the ambiguity of the input.
We further analyze why NDF fails in Appendix~\ref{appendix:baselines}.

Another strength of our method is scalability.
With sparse representation and implicit fields, all of our results process the entire scene as a single input.
On the other hand, previous works~\cite{peng2020conv_onet, chibane20ifnet, chibane2020ndf} process large-scale scenes by cropping them into multiple blocks with sliding window techniques.
This implies that all of the necessary information should be contained in the same block.
Such an assumption fails with severe incompleteness or long-range context.
Being able to observe the rich context of the entire scene, our method produces reasonable completion in various challenging cases.


==> log_likelihood_derivation.tex <==
\section {Derivation of maximizing the log-likelihood}
In this section, we show that the training objective leads to maximizing the marginal log-likelihood of complete data.
We first define a function $G_x(s)$ to ensure the convergence of infusion chain to the complete data distribution:
\begin{equation}
		G_x(s) = \{argmin_{c \in \mathcal{N}(s)}  d(c, c') | c' \in x\}
\end{equation}

Then, we define the infusion chain:
\begin{equation}
    \quad q^t_\phi(s^{t+1} | s^t, x) = \prod_{c \in \mathcal{N}(s^t)} (1 - \alpha^t) p_\phi(c | s^t) + \alpha^t \delta_{G_x(s^t)}(c)
\end{equation}

The following lemma proves that the infusion chain converges to the complete data in finite number of steps.

\begin{restatable}{prop}{infusionconvergence} \label{prop:infusion_convergence}
		If infusion rate $\alpha^t$ is increases linearly until reaching maximum value of 1 and every state $s^t$ is non-empty, then there exist $T$ such that $s^T = x$.
	\label{prop1}
\end{restatable}
\begin{proof}
	\vspace{-0.7em}
	The proof is found in the Appendix~\ref{appendix:prop1}.
	\vspace{-0.7em}
\end{proof}

Due to Proposition~\ref{prop:infusion_convergence}, we can find $T$ such that $x = s^T$.
The objective of the generative model is to maximize the data log-likelihood $\log p_\theta(x) = \log p_\theta(s^T)$, however, since the direct optimization of exact log-likelihood is intractable, we show that our training objective maximizes it's variational lowerbound:
\begin{align}
	\log p_\theta(s^T) 
	&\ge \sum_{s^{0: T-1}} q_\phi(s^{0:T-1}|s^T) \log \frac{p_\theta(s^{0:T})}{q_\phi(s^{0:T-1}|s^T)} \\
	&= \log \frac{p(s^0)}{q(s^0)} + \E_{q_\phi}[\log p_\theta(s^T | s^{T - 1})] - \sum_{0 \le t < T - 1} D_{KL}(q_\phi(s^{t + 1} | s^t, s^T) || p_\theta(s^{t + 1} | s^t))) 
	\label{eq:elbo}
\end{align}
where the full derivation is in the Appendix~\ref{section:detailed_derivation}.
Note that the first term of Equation~\ref{eq:elbo} has no trainable parameters and the second term is maximized directly from the training objective.
The following proposition shows that the training objective minimizes the KL divergence term, therefore maximizing the log-likelihood of data distribution.

\begin{restatable}{prop}{maximizinglowerbound} \label{prop:maximizing_lower_bound}
	Let the parameters of $q$ be updated with $\theta$, parameters of $p$, every time $\theta$ is updated.
	If the likelihood for every cell $c \in s^{t + 1}$ increases when updating parameters $\theta$ with $\theta'$, where $s^{t + 1} \sim q_\theta(\cdot | s^t)$, i.e. $ p_{\theta'}(c | s^t) \ge p_{\theta}(c | s^t), \; \forall c \in s^{t+1}$, then the KL-divergence term in equation~\ref{eq:elbo} decreases, i.e. $D_{KL}(q_\theta(s^{t + 1} | s^t, s^T) || p_\theta(s^{t + 1} | s^t)) \le D_{KL}(q_{\theta'}(s^{t + 1} | s^t, s^T) || p_{\theta'}(s^{t + 1} | s^t))$.
\end{restatable}
\begin{proof}
	\vspace{-0.7em}
	The proof is found in the Appendix~\ref{appendix:prop2}.
	\vspace{-0.7em}
\end{proof}

